Theseus: Exploring Efficient Wafer-Scale Chip Design for Large Language Models

The emergence of the large language model~(LLM) poses an exponential growth of demand for computation throughput, memory capacity, and communication bandwidth. Such a demand growth has significantly surpassed the improvement of corresponding chip designs. With the advancement of fabrication and integration technologies, designers have been developing Wafer-Scale Chips~(WSCs) to scale up and exploit the limits of computation density, memory capacity, and communication bandwidth at the level of a single chip. Existing solutions have demonstrated the significant advantages of WSCs over traditional designs, showing potential to effectively support LLM workloads. Despite the benefits, exploring the early-stage design space of WSCs for LLMs is a crucial yet challenging task due to the enormous and complicated design space, time-consuming evaluation methods, and inefficient exploration strategies. To address these challenges, we propose Theseus, an efficient WSC design space exploration framework for LLMs. We construct the design space of WSCs with various constraints considering the unique characteristics of WSCs. We propose efficient evaluation methodologies for large-scale NoC-based WSCs and introduce multi-fidelity Bayesian optimization to efficiently explore the design space. Evaluation results demonstrate the efficiency of Theseus that the searched Pareto optimal results outperform GPU cluster and existing WSC designs by up to 62.8\%/73.7\% in performance and 38.6\%/42.4\% in power consumption for LLM training, while improving up to 23.2$\times$ and 15.7$\times$ for the performance and power of inference tasks. Furthermore, we conduct case studies to address the design tradeoffs in WSCs and provide insights to facilitate WSC designs for LLMs.

==> hpca-template.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% -- DO NOT MODIFY -- %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\author{
  \ifdefined\hpcacameraready
    \IEEEauthorblockN{\hpcaauthors{}}
      \IEEEauthorblockA{
        \hpcaaffiliation{} \\
        \hpcaemail{}
      }
  \else
    \IEEEauthorblockN{\normalsize{HPCA \hpcayear{} Submission
      \textbf{\#\hpcasubmissionnumber{}}} \\
      \IEEEauthorblockA{
        Confidential Draft \\
        Do NOT Distribute!!
      }
    }
  \fi 
}

% Heading and footer for title page
\fancypagestyle{camerareadyfirstpage}{%
  \fancyhead{}
  \renewcommand{\headrulewidth}{0pt}
  \fancyhead[C]{
    \ifdefined\aeopen
    \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}    
    \else
      \ifdefined\aereviewed
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \ifdefined\aereproduced
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \parbox[][0mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
    \fi 
    \fi 
    \fi 
    \ifdefined\aeopen 
      \includegraphics[width=12mm,height=12mm]{ae-badges/open-research-objects.pdf}
    \fi 
    \ifdefined\aereviewed
      \includegraphics[width=12mm,height=12mm]{ae-badges/research-objects-reviewed.pdf}
    \fi 
    \ifdefined\aereproduced
      \includegraphics[width=12mm,height=12mm]{ae-badges/results-reproduced.pdf}
    \fi
  }
  %\fancyfoot[L]{\hpcapubid{} \copyright \hpcayear{} IEEE}
  \fancyfoot[C]{}
}
% Heading and footer for remaining pages
\fancyhead{}
\renewcommand{\headrulewidth}{0pt}
%\fancyhead[C]{\hpcayear{} IEEE International Symposium on
% High-Performance Computer Architecture (HPCA)}



  


==> tables/arch_design_space.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Architecture Parameters}
\label{tab:design_space}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccc}
\hline
Hierarchy                & Architecture Parameters     & Candidate Values             \\ \hline
\multirow{5}{*}{Core}    & Dataflow                    & 0 for ws, 1 for is, 2 for os \\
                         & Buffer Size (KB)            & 32 to 2048, power of 2       \\
                         & Buffer BW (bit/cycle)       & 32 to 2048, power of 2       \\
                         & MAC Number                  & 8 to 2048, power of 2        \\
                         & NoC BW (bit/cycle)          & 32 to 4096, power of 2       \\ \hline
\multirow{6}{*}{Reticle} & Core Array Height           & 8 to 128                     \\
                         & Core Array Width            & 8 to 128                     \\
                         & Inter-Reticle BW (\%NoC BW) & 25, 50, 75, 100              \\
                         & DRAM bandwidth (TB/s)       & 3 to 24                      \\
                         & DRAM size (GB)              & 6 to 40                      \\
                         & DRAM stacking type          & 2D, 3D-stack                 \\ \hline
\multirow{4}{*}{Wafer}   & Integration Style           & Offset Exposure / InFO-SoW   \\
                         & Reticle Array Height        & 4 to 64                      \\
                         & Reticle Array Width         & 4 to 64                      \\
                         & inter-Wafer BW (GB/s)       & 100, 200, 400                \\ \hline
\end{tabular}%
}
\end{table}

==> tables/benchmark.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Benchmark LLMs}
\label{tab:benchmarks}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|ccccc}
\hline
\textbf{NO.} &
  \textbf{Params (B)} &
  \multicolumn{1}{c|}{\textbf{Layers}} &
  \multicolumn{1}{c|}{\textbf{Hidden Size}} &
  \multicolumn{1}{c|}{\textbf{Attn Heads}} &
  \multicolumn{1}{c|}{\textbf{GPU Num}} &
  \textbf{Batch Size} \\ \hline
0-6, 8-10 & 1.7-1008.0 & \multicolumn{5}{c}{from Megatron-LM~\cite{narayanan2021efficient}}                                                           \\ \hline
7    & 175          & \multicolumn{1}{c|}{96}  & \multicolumn{1}{c|}{12288} & \multicolumn{1}{c|}{96}  & \multicolumn{1}{c|}{1k}   & 2048  \\ \hline
11    & 2244.5       & \multicolumn{1}{c|}{192} & \multicolumn{1}{c|}{32k}   & \multicolumn{1}{c|}{256} & \multicolumn{1}{c|}{6k}   & 3072  \\ \hline
12    & 4066.6       & \multicolumn{1}{c|}{192} & \multicolumn{1}{c|}{42k}   & \multicolumn{1}{c|}{432} & \multicolumn{1}{c|}{12k}  & 5500  \\ \hline
13    & 9588.2       & \multicolumn{1}{c|}{195} & \multicolumn{1}{c|}{64k}   & \multicolumn{1}{c|}{512} & \multicolumn{1}{c|}{30k}  & 10000 \\ \hline
14    & 18436.5      & \multicolumn{1}{c|}{240} & \multicolumn{1}{c|}{80k}   & \multicolumn{1}{c|}{620} & \multicolumn{1}{c|}{60k}  & 15000 \\ \hline
15    & 32405.7      & \multicolumn{1}{c|}{270} & \multicolumn{1}{c|}{100k}  & \multicolumn{1}{c|}{850} & \multicolumn{1}{c|}{100k} & 20000 \\ \hline
\end{tabular}%
}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \begin{table}[]
% \centering
% \caption{Benchmark LLMs}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{ccccc}
% \hline
% Model Scale & Params & Layers & Hidden Size & Attn Heads \\ \hline
% Small       & 1.7B   & 24     & 2304        & 24         \\ \hline
% Medium      & 175B   & 96     & 12288       & 96         \\ \hline
% Large       & 530B   & 105    & 20480       & 128        \\ \hline
% \end{tabular}%
% }
% \label{tab:benchmarks}
% \end{table}



==> tables/llm_tasks.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ll|l|l|l|l}
\hline
\multicolumn{2}{l|}{}                        & Comp Power & Comm Bandwidth & Mem Capacity & Mem Bandwidth             \\ \hline
\multicolumn{2}{l|}{Training}                 & \checkmark & \checkmark & \checkmark & - \\ \hline
\multicolumn{2}{l|}{Inference(Prefill stage)} & \checkmark & \checkmark & \checkmark & - \\ \hline
\multicolumn{2}{l|}{Inference(Decode stage)} & -          & -              & -            & \checkmark \\ \hline
\end{tabular}%
}
\caption{LLM Training and Inference Requirements}
\label{tab:llm_tasks}
\end{table}

==> tables/parallel_design_space.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\Huge
\caption{Parallel Strategy Design Space}
\label{tab:pa_design_space}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccc}
\hline
Parallel Parameters & Candidate Values                & Constraints                                \\ \hline
DP size &
  $\mid$ Wafer num &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}DP size $\times$ PP size $\leq$ wafer num\\ microbatch size $\times$ DP size $\leq$ batch size\end{tabular}} \\ \cline{1-2}
PP size             & $\mid$ Layer num          &                                             \\ \cline{1-2}
microbatch size     & $\mid$ batch size            &                                             \\ \hline
TP size             & $\mid$ att\_head num & TP size $\leq$ reticle per wafer \\ \hline
\end{tabular}%
}
\end{table}

==> tex/discussion.tex <==
\section{Discussion}

Exposed / Overlapped communication

Communication bandwidth / Memory Bandwidth (Capacity) tradeoff
